Spin-dependent phenomena at chiral temporal interfaces

Temporally varying electromagnetic media have been extensively investigated recently to unveil new means for controlling light. However, spin-dependent phenomena in such media have not been explored thoroughly. Here, we reveal the existence of spin-dependent phenomena at a temporal interface between chiral and dielectric media. In particular, we show theoretically and numerically that due to the material discontinuity in time, linearly polarized light is split into forward-propagating right-handed and left-handed circularly polarized waves having different angular frequencies and it the same phase velocities. This salient effect allows complete temporal separation of the two spin states of light with high efficiency. In addition, a phenomenon of spin-dependent gain/loss is observed. Furthermore, we show that when the dielectric medium is switched again to the original chiral medium, the right- and left-handed circularly polarized light waves (with different angular frequencies) merge to form a linearly polarized wave. Our findings extend spin-dependent interactions of light from space to space-time.

==> nature-bib.tex <==
\begin{thebibliography}{9}

%\bibitem{MSMNM}
%M.S.~Mirmoosa, T.T.~Koutserimpas, G.A.~Ptitcyn, S.A.~Tretyakov, \& R.~Fleury, ``Dipole polarizability of time-varying particles," {\itshape arXiv:2002.12297} (2020). 

%\bibitem{Engheta} 
%D.M.~Sol{\'i}s \& N.~Engheta, ``Functional analysis of the polarization response in linear time-varying media: A generalization of the Kramers-Kronig relations," {\itshape Phys.~Rev.~B} 103, 144303 (2021). 

\bibitem{review} 
Shaltout, A. M., Shalaev, V. M., \& Brongersma, M. L. Spatiotemporal light control with active metasurfaces. {\itshape Science} 364, 6441 (2019).

\bibitem{Fang} 
Fang, K., Luo, J., Metelmann, A. et al. Generalized non-reciprocity in an optomechanical circuit via synthetic magnetism \& reservoir engineering. {\itshape Nature Physics} 13, 465–471 (2017).

\bibitem{bi}
Wang, X., Ptitcyn, G., Asadchy, V. S., D\'{\i}az-Rubio, A., Mirmoosa, M. S., Shanhui, F. \& Tretyakov, S.A. Nonreciprocity in Bianisotropic Systems with Uniform Time Modulation. {\itshape Phys. Rev. Lett.} 125, 26 (2020).

\bibitem{nonrec-rev}
Sounas, D. L., Alù, A. Non-reciprocal photonics based on time modulation. {\itshape Nature Photonics} 11, 774–783 (2017).

\bibitem{luminal}
Galiffi, E., Huidobro, P. \& Pendry, J. Broadband Nonreciprocal Amplification in Luminal Metamaterials. {\itshape Phys. Rev. Lett.} 123, 206101 (2019).

\bibitem{Huanan}
Li, H., Yin, S. \& Alù, A. {\itshape Phys. Rev. Lett.} 128, 173901 (2022).

\bibitem{Lee}
Lee, K., Son, J., Park, J. et al. Linear frequency conversion via sudden merging of meta-atoms in time-variant metasurfaces. {\itshape Nature Photonics} 12, 765–773 (2018).

\bibitem{Liu}
Liu, M., Powell, D., Zarate, Y. \& Shadrivov, I. Huygens’ Metadevices for Parametric Waves. {\itshape Phys. Rev. X} 8, 031077 (2018).

\bibitem{Shaltout}
Shaltout, A. M. et al. Spatiotemporal light control with frequency gradient metasurfaces.  {\itshape Science} 365(6451), 374–377 (2019).

\bibitem{Bacot} 
Bacot, V., Labousse, M., Eddi, A. et al. Time reversal \& holography with spacetime transformations. {\itshape Nature Physics} 12, 972–977 (2016).

\bibitem{Pacheco} 
Pacheco-Peña, V. \& Engheta, N. Antireflection temporal coatings. {\itshape Optica} 7, 323-331 (2020).

\bibitem{PendryRev} 
Galiffi, E. et al. Photonics of time-varying media. {\itshape Advanced Photonics} 4, 014002 (2022).

%\bibitem{nonrec}
%X. Guo, Y. Ding, Y. Duan,  X. Ni, ``Nonreciprocal metasurface with space–time phase modulation," {\itshape Light Sci Appl} 8, 123 (2019). 

%\bibitem{extreme energy}
%M.S. Mirmoosa, G.A. Ptitcyn, V.S. Asadchy, \& S.A. Tretyakov, ``Time-Varying Reactive Elements for Extreme Accumulation of Electromagnetic Energy," {\itshape Phys. Rev. Applied,} 11, 1 (2019).

\bibitem{temporalaiming}
Pacheco-Peña, V., Engheta, N. Temporal aiming. {\itshape Light Sci Appl,} 9, 129 (2020).

\bibitem{Akbarzadeh}
Akbarzadeh A., Chamanara, N. \& Caloz, C. Inverse prism based on temporal discontinuity \& spatial dispersion. {\itshape Opt. Lett.} 43, 3297-3300 (2018).

%\bibitem{Huanan}
%Li, H., Yin, S., \& Alù, A. Nonreciprocity \& Faraday Rotation at Time Interfaces. {\itshape Phys. Rev. Lett.} 128, 173901 (2022).

\bibitem{Huidobro}
Huidobro, P. A. et al. Fresnel drag in space–time-modulated metamaterials. {\itshape Proc. Natl. Acad. Sci.} 116(50), 24943–24948 (2019).

\bibitem{Huidobro2}
Huidobro, P. A. et al. Homogenization theory of space-time metamaterials. {\itshape Phys. Rev. Appl.} 16(1), 014044 (2021).

\bibitem{Fortuno}
Bliokh, K., Rodríguez-Fortuño, F., Nori, F. et al. Spin–orbit interactions of light. {\itshape Nature Photonics} 9, 796–808 (2015). 

\bibitem{Aiello}
Aiello, A., Banzer, P., Neugebauer, M. et al. From transverse angular momentum to photonic wheels. {\itshape Nature Photonics} 9, 789–795 (2015). 

\bibitem{Shi}
Shi, P. et al. Transverse spin dynamics in structured electromagnetic guided waves. {\itshape Proc. Natl. Acad. Sci.} 118(6), e2018816118
(2021).

\bibitem{Eismann}
Eismann, J. S., Nicholls, L. H., Roth, D. J. et al. Transverse spinning of unpolarized light. {\itshape Nature Photonics} 15, 156–161 (2021). 

\bibitem{Chen}
Chen, P. et al. Chiral Coupling of Valley Excitons \& Light through Photonic Spin–Orbit Interactions. {\itshape Adv. Funct. Mater.} 8, 5 (2019). 

\bibitem{Higo}
Higo, T., Man, H., Gopman, D. B. et al. Large magneto-optical Kerr effect \& imaging of magnetic octupole domains in an antiferromagnetic metal. {\itshape Nature Photonics} 12, 73–78 (2018).

\bibitem{spin}
Onoda, M., Murakami, S. \& Nagaosa, N. Hall effect of light. {\itshape Phys. Rev. Lett.} 93, 083901 (2004).

\bibitem{Bliokh}
Bliokh, K. \& Bliokh, P. Topological spin transport of photons: the optical Magnus effect \& Berry phase. {\itshape Physics Letters A.} 333, 3–4 (2004).

\bibitem{Hosten}
Hosten, O. \& Kwiat, P. Observation of the Spin Hall Effect of Light via Weak Measurements. {\itshape Science} 319, 5864 (2008).

\bibitem{Zhou}
Zhou, X., Xiao, Z., Luo, H. \& Wen, S. Experimental observation of the spin
Hall effect of light on a nanometal film via weak measurements. {\itshape Phys. Rev. A} 85, 043809 (2012).

\bibitem{Ari}
Lindell, I. V., Sihvola, A. H., Tretyakov, S. A. \& Viitanen, A. J. Electromagnetic Waves in Chiral \& Bi-isotropic Media. {\itshape Norwood, MA: Artech House}, (1994).

\bibitem{CONDON}
Condon, E. U., Altar, W. \& Eyring, H. One‐Electron Rotatory Power. {\itshape J. Chem. Phys.} 5, 753 (1937).

\bibitem{Morgen}
Morgenthaler, F. Velocity Modulation of Electromagnetic Waves. {\itshape IEEE Trans. Microw. Theory Tech.} 6, 167 (1958).

\bibitem{Serdyukov}
Serdyukov, A. N. Semchenko, I. V.,  Tretyakov, S. A. \& Sihvola, A. H. Electromagnetics of bi-anisotropic materials: Theory and applications, {\itshape Amsterdam: Gordon and Breach Science Publishers}, (2001).

\bibitem{JEWA}
Tretyakov, S. T. \& Mariotte, F. Maxwell Garnett modeling of uniaxial chiral composites with bianisotropic inclusions, {\itshape Journal of Electromagnetic Waves and Applications}, vol. 9, no. 7/8, pp. 1011-1025, (1995).

%C. Caloz \& A. Sihvola, ``Electromagnetic Chirality, Part 2: The Macroscopic Perspective [Electromagnetic Perspectives]," {\itshape IEEE Antennas \& Propagation Magazine,} vol. 62, no. 2, pp. 82-98, (2020).




\end{thebibliography}


